One Picture is Worth a Thousand Words: A New Wallet Recovery Process

We introduce a new wallet recovery process. Our solution associates 1) visual passwords: a photograph of a secretly picked object (Chabanne et al., 2013) with 2) ImageNet classifiers transforming images into binary vectors and, 3) obfuscated fuzzy matching (Galbraith and Zobernig, 2019) for the storage of visual passwords/retrieval of wallet seeds. Our experiments show that the replacement of long seed phrases by a photograph is possible.

==> fig.tex <==
\begin{figure*}\centering
\begin{tikzpicture}[mylabel/.style={text width=8 mm, align=center}]
\node[bob, minimum width=1.5cm, 
%   label={[mylabel, anchor=west]north east:{Public\\ n, e}},
%    label={[mylabel, anchor=east]north west:{Private\\ d}}
    ] (bob) {1. $U$ picks his visual password $c$};
\node[conductor, minimum width=1.5cm, right=5cm of bob, mirrored,
%    label={[mylabel, anchor=east]north west:{Public}}, 
%    label={[mylabel, anchor=west]north east:{Private\\ M}}
    ] (alice) {};

\draw[->, thick] ([yshift=2mm]bob.east) coordinate(aux-a)-- coordinate[near start] (aux) node[above, text width=1.5cm, align=center]{\mbox{\hspace{-1.4cm}  2. $U$ stores ENCODE(c) (\ref{encode})}}  (aux-a-|alice.west);
\end{tikzpicture}
\caption{Visual Password Storage}
\label{fe}
\end{figure*}


\begin{figure*}\centering
\begin{minipage}{12cm}\centering 
\begin{tikzpicture}[mylabel/.style={text width=8 mm, align=center}]
\node[bob, minimum width=1.5cm, 
%   label={[mylabel, anchor=west]north east:{Public\\ n, e}},
%    label={[mylabel, anchor=east]north west:{Private\\ d}}
    ] (bob) {\begin{minipage}{16.5cm}\raggedleft 
    \begin{tabular}{l}
       3. $U$ captures $x$ a new image of his visual password \\ 3bis. $U$ retrieves his wallet's seed as RETRIEVESEED(ENCODE($c$),$x$)

    \end{tabular}
\end{minipage}};
\node[conductor, minimum width=1.5cm, right=5cm of bob, mirrored,
    ] (alice) {};

\draw[->, thick] ([yshift=2mm]bob.east) coordinate(aux-b)-- node[above, text width=1.5cm, align=center]{\mbox{\hspace{-1.9cm} 1. $U$ asks for his visual password}} coordinate[near end] (auxtwo) (aux-b-|alice.west);

\draw[<-, thick] ([yshift=-3mm]bob.east) coordinate(aux-a)-- coordinate[near start] (aux) node[above, text width=1.5cm, align=center]{\mbox{\hspace{-1cm} 2. ENCODE($c$)}} (aux-a-|alice.west);
\end{tikzpicture}
\end{minipage}
\vspace{1cm}
\caption{Wallet's Seed Retrieval}
\label{fa}
\end{figure*}
